GOFA: A Generative One-For-All Model for Joint Graph Language Modeling

Foundation models, such as Large Language Models (LLMs) or Large Vision Models (LVMs), have emerged as one of the most powerful tools in the respective fields. However, unlike text and image data, graph data do not have a definitive structure, posing great challenges to developing a Graph Foundation Model (GFM). For example, current attempts at designing general graph models either transform graph data into a language format for LLM-based prediction or still train a GNN model with LLM as an assistant. The former can handle unlimited tasks, while the latter captures graph structure much better -- yet, no existing work can achieve both simultaneously. In this paper, we identify three key desirable properties of a GFM: self-supervised pretraining, fluidity in tasks, and graph awareness. To account for these properties, we extend the conventional language modeling to the graph domain and propose a novel generative graph language model GOFA to solve the problem. The model interleaves randomly initialized GNN layers into a frozen pre-trained LLM so that the semantic and structural modeling abilities are organically combined. GOFA is pre-trained on newly proposed graph-level next-word prediction, question-answering, and structural tasks to obtain the above GFM properties. The pre-trained model is further fine-tuned on downstream tasks to obtain task-solving ability. The fine-tuned model is evaluated on various downstream tasks, demonstrating a strong ability to solve structural and contextual problems in zero-shot scenarios. The code is available at https://github.com/JiaruiFeng/GOFA.

==> tab/data_abla.tex <==
\begin{table}[]
\begin{tabular}{@{}llll@{}}
\toprule
 & FB15K237 & Products & Cora-Link \\ \midrule
Full & 73.82 & 82.15 & 77.45 \\
w/o R & 57.81 & 78.29 & 72.91 \\
w/o R+W  & 55.96 & 75.83 (?) & 65.91 (?)\\ \bottomrule
\end{tabular}
\end{table}

==> tab/diff_prompt_examples.tex <==
% \begin{tabular}{p{5cm}|p{9cm}}
% \toprule
% \includegraphics[width=5cm]{figs/diff_prompt_fig1.pdf} &
% \vspace{-10pt} Answer: Based on the papers \\ \midrule
% \includegraphics[width=5cm]{figs/diff_prompt_fig2.pdf} &
% Answer: The core concept \\ \midrule
% \includegraphics[width=5cm]{figs/diff_prompt_fig3.pdf} &
% Answer: The shortest path  \\ 
% \bottomrule
% \end{tabular}
\begin{table}[t]
    \begin{center}
        \begin{tabular}{c p{9cm}}
        \toprule
        \raisebox{-\totalheight}{\includegraphics[width=0.3\textwidth]{figs/diff_prompt_fig1.pdf}} & Answer: \newline Based on the papers you have provided, here are some potential research ideas: 
1. Adversarial attacks on generative models: The paper "Adversarial Examples in the Physical World" demonstrates that adversarial examples can be crafted in real-world settings. Could this concept be extended to generative models, such as GANs, to create adversarial examples capable of deceiving these models? 
2. Generative models for drug discovery ... \\ \midrule
\raisebox{-\totalheight}{\includegraphics[width=0.3\textwidth]{figs/diff_prompt_fig2.pdf}} & Answer: \newline The core concept of these papers is the application of GANs to generate realistic images. The first paper introduces a new loss function for GANs that incentivizes the generator to create images that closely resemble real ones, rather than merely aligning with those judged as similar by the discriminator. The second paper... \\ \midrule
\raisebox{-\totalheight}{\includegraphics[width=0.3\textwidth]{figs/diff_prompt_fig3.pdf}} & Answer: \newline The shortest path distance is 3. The shortest paths between [NODE.F] and [NODE.H] are : [NODE.F] $\rightarrow$ [NODE.X] $\rightarrow$ [NODE.K] $\rightarrow$ [NODE.G] and [NODE.F] $\rightarrow$ [NODE.Z] $\rightarrow$ [NODE.S] $\rightarrow$ [NODE.G].  \\ 
\bottomrule
        \end{tabular}
    \end{center}
\end{table}
% \begin{tabular}{c|p{9cm}}
% \toprule
% \includegraphics[width=5cm]{figs/diff_prompt_fig1.pdf} &
% \raisebox{-10mm}{Answer: Based on the papers you have provided, here are some potential research ideas: 
% 1. Adversarial attacks on generative models: The paper "Adversarial Examples in the Physical World" demonstrates that adversarial examples can be crafted in real-world settings. Could this concept be extended to generative models, such as GANs, to create adversarial examples capable of deceiving these models? 
% 2. Generative models for drug discovery ...}  \\ \midrule
% \includegraphics[width=5cm]{figs/diff_prompt_fig2.pdf} &
% Answer: The core concept of these papers is the application of generative adversarial networks (GANs) to generate realistic images. The first paper introduces a new loss function for GANs that incentivizes the generator to create images that closely resemble real ones, rather than merely aligning with those judged as similar by the discriminator. The second paper... \\ \midrule
% \includegraphics[width=5cm]{figs/diff_prompt_fig3.pdf} &
% Answer: The shortest path distance is 3. Shortest paths: [NODEID.F] -> [NODEID.X] -> [NODEID.K] -> [NODEID.G]. \\ 
% \bottomrule
% \end{tabular}

% \begin{table}[h!]
%      \begin{center}
%      \begin{tabular}{ c  p{5cm}  p{5cm}  }
%      \toprule
%       my.Lboro & Advantages & Disadvantages \\ 
%     \cmidrule(r){1-1}\cmidrule(lr){2-2}\cmidrule(l){3-3}
%      \raisebox{-\totalheight}{\includegraphics[width=0.3\textwidth, height=60mm]{figs/diff_prompt_fig1.pdf}}
%       & 
%       \begin{itemize}[topsep=0pt]
%       \item Accessibility
%       \item Up to date information
%       \item Fulfil students needs and wants \ldots
%       \end{itemize}
%       & 
%       \begin{itemize}[topsep=0pt]
%       \item Accessibility
%       \item Up to date information
%       \item Fulfil students needs and wants \ldots
%       \end{itemize}
%       \\ \bottomrule
%       \end{tabular}
%       \caption{my.Lboro Analysis}
%       \label{tbl:myLboro}
%       \end{center}
% \end{table}

% \begin{figure}[h]
%   \centering
%   \begin{minipage}[t]{0.3\textwidth}
%     \centering
%     \includegraphics[width=4cm]{figs/diff_prompt_fig.pdf} % Adjust height
%     \caption{Figure}
%   \end{minipage}
%   \hfill
%   % Create a minipage for the table
%   \begin{minipage}[t]{0.6\textwidth}
%     \centering
%     \begin{tabular}{p{7.5cm}}
%     \toprule
%     % Prompt: Given these papers, please creatively think about some research ideas. \\ 
%     Answer: Based on the papers you have provided, here are some potential research ideas: \newline
%     1. Adversarial attacks on generative models: The paper "Adversarial Examples in the Physical World" demonstrates that adversarial examples can be crafted in real-world settings. Could this concept be extended to generative models, such as GANs, to create adversarial examples capable of deceiving these models? \newline
%     2. Generative models for drug discovery ... \\ \midrule
%     % Prompt: Please summarize the core concept of these papers. \\ 
%     Answer: The core concept of these papers is the application of generative adversarial networks (GANs) to generate realistic images. The first paper introduces a new loss function for GANs that incentivizes the generator to create images that closely resemble real ones, rather than merely aligning with those judged as similar by the discriminator. The second paper... \\ \midrule
%     % Prompt: Please compute the shortest path distance between node [NODE.II] and [NODE.YM] and generate all shortest paths from [NODE.II] to [NODE.YM]. \\ 
%     Answer: The shortest path distance is 3. Shortest paths: [NODEID.F] -> [NODEID.X] -> [NODEID.K] -> [NODEID.G]. \\ 
%     \bottomrule
%     \end{tabular}
%   \end{minipage}

% \end{figure}


==> tab/prompt_edge.tex <==
\begin{wrapfigure}[7]{R}{0.42\textwidth}
\small
\setlength{\tabcolsep}{5.0pt}
\begin{minipage}[t]{0.95\linewidth}
\captionsetup{type=table}

\caption{Ablation study on prompt edge.}
\label{tab:abla}
\vspace{-3pt}
\begin{tabular}{@{}ccc@{}}

\toprule
 & Single Edge & Double Edge \\ \midrule
Cora-Link & 49.6 & 59.4 \\
Cora-Node & 58.6 & 60.2 \\
Products & 2.8 & 22.8 \\ \bottomrule
\end{tabular}
\end{minipage}

\end{wrapfigure}


==> tab/zero_shot_link.tex <==
% \begin{wraptable}[15]{r}{0.40\linewidth}
% \vspace{-20pt}
% \small
% \setlength{\tabcolsep}{4.0pt}
% \label{tab:abla}
% \begin{minipage}[t]{0.95\linewidth}
% \setlength{\tabcolsep}{1pt}
%     \caption{PubMed link instruction tuning on zero-shot setting (Accuracy).}
% \small
% \begin{tabular}{@{}ccc@{}}

% \toprule
%  Model & Cora-Link \\
%  Way   &     2     \\
% \midrule
% \midrule
% Llama2-7B & 49.72  \\
% Mistral-7B & 41.34 \\
% % Llama2-13B & - & - \\
% \midrule
% OFA-Llama2 & 52.22  \\
% \midrule
% \textbf{GOFA-Llama2-Pubmed} & \underline{62.36} \\
% \textbf{GOFA-Mistral-Pubmed} & \textbf{64.8} \\
% \bottomrule
% \end{tabular}
% \end{minipage}

% 
%\end{wraptable}
\begin{wraptable}[12]{R}{0.35\textwidth}
\vspace{-10pt}
\caption{PubMed link instruction tuning on zero-shot setting (Acc).}
\label{tab:comparison}
\small
\centering
\setlength{\tabcolsep}{1pt}
\hspace{-5pt}
\begin{tabular}{@{}cc@{}}
\toprule
 Task & Cora-Link \\
 Way   &     2     \\
\midrule
\midrule
Llama2-7B & 49.72  \\
Mistral-7B & 41.34 \\
% Llama2-13B & - & - \\
\midrule
OFA-Llama2 & 52.22  \\
\midrule
\textbf{GOFA-Llama2-Pubmed} & \underline{62.36} \\
\textbf{GOFA-Mistral-Pubmed} & \textbf{65.91} \\
\bottomrule
\end{tabular}
\vspace{-20pt}
\end{wraptable}

==> tab/zero_shot_mol.tex <==
\begin{wraptable}[10]{R}{0.28\linewidth}
\vspace{-12pt}
\small
%\setlength{\tabcolsep}{2.0pt}
\begin{minipage}[t]{0.8\linewidth}
\caption{Zero-shot learning with molecule dataset}
\vspace{-7pt}
\label{tab:zero_shot_mol}
\begin{tabular}{@{}ccc@{}}
\toprule
& BBBP& HIV \\ \midrule
OFA   &   -   &  35.67 \\
MoMu   &   49.81   &  50.26 \\
Galactica & 53.94 & 33.85 \\
GIMLET &  59.39 & 66.24 \\
GOFA &  54.91  &  53.02 \\
\bottomrule
\end{tabular}
\end{minipage}
% % \begin{minipage}[t]{0.9\linewidth}
% \begin{minipage}[t]{0.95\linewidth}
% \vspace{-1pt}
% \centering
%     \includegraphics[width=0.92\textwidth, trim={0.2cm 0.2cm 1.5cm 1.0cm}, clip]{figs/llama_loss.pdf}
% \vspace{-6pt}
% \captionsetup{type=figure}
% \caption{GOFA training loss.}
% \label{fig:loss}

% \end{minipage}

\end{wraptable}

==> tab/zero_shot_ppi.tex <==
\begin{wraptable}[7]{R}{0.25\linewidth}
\vspace{-12pt}
\small
%\setlength{\tabcolsep}{2.0pt}
\begin{minipage}[t]{0.85\linewidth}
\caption{Zero-shot learning on PPI dataset}
\vspace{-7pt}
\label{tab:zero_shot_ppi}
\begin{tabular}{@{}cc@{}}
\toprule
 Model & AUROC\\ \midrule
Mistral-7B  &  35.24 \\
GOFA-T   &   64.59 \\
\bottomrule
\end{tabular}
\end{minipage}
% % \begin{minipage}[t]{0.9\linewidth}
% \begin{minipage}[t]{0.95\linewidth}
% \vspace{-1pt}
% \centering
%     \includegraphics[width=0.92\textwidth, trim={0.2cm 0.2cm 1.5cm 1.0cm}, clip]{figs/llama_loss.pdf}
% \vspace{-6pt}
% \captionsetup{type=figure}
% \caption{GOFA training loss.}
% \label{fig:loss}

% \end{minipage}

\end{wraptable}

==> tex/outline.tex <==
\textbf{Introduction}

\begin{enumerate}
    \item Foundation models become a powerful tool. (Versatility, interpretability, universality etc.)
    \item Direct application of llm fails on graph problem. (Missing structural awareness, no reliable protocol to take in graph data.)
    \item A series of \textit{General} Graph Models emerges with the ability to handle a broader range of tasks than a single GNN. Mention iconic works.
    \item Discuss the drawbacks of existing approaches. Should be linked to the graph foundation model that we propose.
    \item Inspired by LLM, we identify desirable attributes of a graph foundation model.
    \item We then propose a probabilistic formulation of the graph foundation modeling problem. By solving the problem, users can query arbitrary nodes with tasks such as sentence completion and question answering just like in using LLMs.
    \item We propose a Graph Language Model that solves the proposed problem. The model interleaves new token-level GNN layers into frozen LLM layers. The LLM layers compress node sentences into vector representations of fixed length, and the GNN layers facilitate message-passing between compressed graph node representations. Eventually, we use an LLM to generate texts based on the structural and semantic information stored in the graph node representations.
    \item Experiement
\end{enumerate}

\textbf{Graph Foundation Model}

This section should contain just enough information and subject to deduction and moved to appendix. Discuss desirable properties of the graph foundation model

\begin{enumerate}
    \item GFM is important because LLM can't handle relational data well.
    \item Existing GNN/Graph transformers are not foundational architecture.
    \item GFM should be both good at what LLM is good at and good at what GM is good at.
    \item Properties:
    \begin{itemize}
        \item Unsupervised Large-scale pertaining  ---> lead to universal/transferrable model
        \item Fluidity in task. Even should not be limited to Generation/Classification/Regression, but should be able to do arbitrary tasks, as long as we have training data. ---> lead to language output as endpoint.
        \item In-context learning   ---->    prompting should not be limited to text level, but to graph level.
        \item Ability to comprehend graph structural information   ---->   with good expressivity which is where LLM falls short on
    \end{itemize}
\end{enumerate}

\textbf{Approach}
\begin{enumerate}
    \item Next word prediction like modeling formulation. Why a model that solves this modeling problem serves well as a graph foundation model ----> link to our GFM attribute.
    \item To solve such a problem, we need a model architecture that can transform text in graphs into continuous representations, which LLM does well. 
    \item We also need a graph model that combines text information on different nodes via edges/connections in graph. Because a sentence is represented by multiple tokens, the GNN needs to handle message passing between sequence of tokens.
    \item Sentences are different in length as well as the token representation, but GNN takes only fixed length input. We propose to use a sentence compressor to compress full sentence information into a fixed-length sequence representation.
    \item The overall architecture interleaves GNN into pretrained frozen LLM sentence compressor, the compressed node texts tokens and edge texts tokens are used to generate new node text representations. The texts tokens are directly fed to the next LLM layer. The GNN output are controlled by a trainable tanh gate. Add residual and ff.
    \item Any node representations cover neighboring semantic information as well as structural information. We use a language tokens to generate text based on the node representations. With examples.
\end{enumerate}

\textbf{Training GGM on diverse graph datasets}
\begin{enumerate}
    \item Implementation
    \begin{itemize}
        \item In actual implementation, last t layers are interleaved with GNN.
        \item A trained LLM auto-encoder fit the scenario well, and we use ICAE as the LLM encoder. But we can extend to arbitrary compressor given small tweak in model architecture. \textit{potentially propose several use models like mamba.}
    \end{itemize}
    \item Node-level Sentence completion task, relevance to causal LM training. Focus on unsupervised nature and use neighbor nodes to enhance LLM understanding of node information.
    \item Question Answering
    \begin{itemize}
        \item Content QA: link prediction. focus on graph specific task.
        \item Structural QA: graph structural learning
        \item Chain of QA: explain graph tasks are limited, regular QA also helps understanding of the problem.
    \end{itemize}
\end{enumerate}

\textbf{Experiment}
